A Challenging Benchmark for Low-Resource Learning

With promising yet saturated results in high-resource settings, low-resource datasets have gradually become popular benchmarks for evaluating the learning ability of advanced neural networks (e.g., BigBench, superGLUE). Some models even surpass humans according to benchmark test results. However, we find that there exists a set of hard examples in low-resource settings that challenge neural networks but are not well evaluated, which causes over-estimated performance. We first give a theoretical analysis on which factors bring the difficulty of low-resource learning. It then motivate us to propose a challenging benchmark hardBench to better evaluate the learning ability, which covers 11 datasets, including 3 computer vision (CV) datasets and 8 natural language process (NLP) datasets. Experiments on a wide range of models show that neural networks, even pre-trained language models, have sharp performance drops on our benchmark, demonstrating the effectiveness on evaluating the weaknesses of neural networks. On NLP tasks, we surprisingly find that despite better results on traditional low-resource benchmarks, pre-trained networks, does not show performance improvements on our benchmarks. These results demonstrate that there are still a large robustness gap between existing models and human-level performance.

==> 03.1_pre.tex <==







% For a better description, we introduce the notations used in this paper. Let $\mathcal{X}$ be the data space, $\mathcal{Y}$ be the label space, and $\mathcal{H}$ be the hypothesis space in our investigation $\mathcal{H}: \mathcal{X}\rightarrow\mathcal{Y}$. We consider classification tasks for simplification. %Under this setting, an algorithm has access to a 
% The training set $X$ consists of $n$ samples $(x_i, y_i)_{i=1}^n\sim P(X,Y) $. The model $f_{\theta}\in \mathcal{H}$ maps input to prediction $Y\in \mathbbm{R}^d$, where $d$ denotes the dimensions of the output and $\theta$ represents the parameters of the model. To give a probabilistic view of the problem, the training distribution is denoted as $P(X, Y) = \frac{1}{n}\sum_{i=1}^n \delta_{(x_i,y_i)}$, where $\delta$ denotes the Dirac delta distribution concentrated on $(x_i,y_i)$. Consequently, $P(X) = \frac{1}{n}\sum_{i=1}^n \delta_{x_i}$ and $P(Y) = \frac{1}{n}\sum_{i=1}^n \delta_{y_i}$. 



==> 03.2_def.tex <==






% In this work, we discuss the problem of few-shot robustness. In traditional few-shot learning, we construct a few-shot set and measure the performance given the fixed training set and test set. Here we are interested in if different few-shot training sets lead to large model performance degradation. Inspired by the notion of robustness in distributional robust optimization \citep{sagawa2019distributionally,kuhn2019wasserstein}, we aim to find a challenging few-shot training set 
% $P_{\text{few}}$ that maximizes the expected risk on the test set. For convenience, we focus on a data-driven few-shot distribution, where $P_{\text{few}}$ is centered around empirical examples extracted from the original training set distribution. 

% We consider a few shot set with $k$ examples. The example index is defined as ${I}_k := \{i_1, i_2, ... i_k\}\subset[n]$, and therefore $P_{\text{few}}(X)=\frac{1}{k}\sum_{m=1}^k \delta_{X_{i_m}}$. For short, we also write $P_{\text{few}}(X)$ as $P_{{I}_k}(X)$. Let $f$ be the model hypothesis and $Q$ as the test distribution, the empirical risk of $f$ w.r.t training set $P$ is $\epsilon_P(f) = \mathbbm{E}_{x\in P(x)}|\delta(f(x)) - P(y|x)|$, and the expected risk of $f$ w.r.t. $Q$ is denoted as $\epsilon_Q(f) = \mathbbm{E}_{x\in Q(x)}|\delta(f(x)) - Q(y|x)|$. We assume the original training sets and test sets are sampled $i.i.d$ from a natural distribution. Then we can safely make Assumption.~\ref{generalization} that the full-size training set can teach a model with acceptable generalization errors. %the original training set can be successfully generalized to the test set. 

% \begin{assumption}\label{generalization}\textit{(Generalization)} 
% Let $\mathcal{H}: X \rightarrow Y $ be the hypothesis space, then there exists a model $f$ satisfies $f\in \mathcal{H}$ and $\epsilon_P(f)\leq \alpha$, $\epsilon_Q(f)\leq \beta$, where $\alpha$, $\beta$ are constants approaching zero.
% \end{assumption}

% In a real-world setting, a few-shot dataset is usually constructed by choosing a few representative samples~\citep{parnami2022learning, gao2020making}. Data imbalance is preferably avoided so as not to inject bias~\citep{ochal2021few, DBLP:journals/csur/WangYKN20}. It is thus logical to assume that the few-shot subset should match the balanced label distribution of the original training set, as stated in Assumption.~\ref{label alignment}. 
% %in order to teach the model the problem settings. 
% %For the classification problem, a logical way is to sample a few training samples for each class \citep{parnami2022learning, gao2020making}. 


% \begin{assumption}\label{label alignment}\textit{(Label Alignment)} 
% Let $P_{I_k}(X,Y)$ be the few-shot set selected from $P(X,Y)$, then $I_k$ should satisfy $P(Y) = P_{\text{few}}(Y)$, i.e, $\frac{1}{n}\sum_{i=1}^n\delta_{Y_{i}} = \frac{1}{k}\sum_{m=1}^k\delta_{Y_{i_m}} $. 
% \end{assumption}


% \paragraph{Few-shot Robustness} Under these assumptions, the few-shot robustness problem we address asks to solve the worst-case problem denoted as,
% \begin{equation}\label{main def}
%     \max_{{I}_k   
%     } \epsilon_Q(f_{I_k}),
% \end{equation}
% where $f_{I_k}$ is a hypothesis that satisfies $\epsilon_{P_{{I}_k}}(f_{I_k})\leq \alpha $, and ${I}_k $ satisfies $\frac{1}{n}\sum_{i=1}\delta_{Y_{i}} = \frac{1}{k}\sum_{}\delta_{Y_{i,m}} , i\in [n], m\in {I}_k,  {I}_k\subset[n] $ . $\{P_{I_k}\}$ is the uncertainty set for constraining this distributional robustness problem. Different few-shot training sets $X_{{I}_k}$ lead to varied generalization errors. 

% Traditional few-shot evaluation usually adopts a fixed training set. Correlations between the training set and the test set largely decide the generalization errors on the test set. Higher performance does not represent better robustness due to the missing evaluation of the worst-case performance. To evaluate few-shot robustness in Eq.~\ref{main def}, the target is to find a subset $X_{{I}_k}$ to prevent models from learning biased features and increase the difficulty for generalization performance. 

==> 04_preliminaries.tex <==


% This section introduces our method for evaluating the worst-case generalization error by constructing a challenging few-shot set based on Eq.~\ref{main def}. The intuition of NMMD-ATTACK is based on eliminating the spurious correlation between few-shot training set and test set. Since most samples hold spurious attributes \citep{sagawa2019distributionally} and samples with the same spurious attributes tend to be more similar, it is more likely to find less biased subsets based on distribution discrepancy. Therefore, we propose a \method approach to find the worst-case few-shot subset with the largest MMD discrepancy from the original training distribution, while maintaining the balance of labels.  

% Here, We first proves the intuition that the worst-case can be achieved by maximizing the MMD distance between few-shot set and the original training set, and then introduce how to quantitatively evaluate the MMD distance using neural tangent kernel. Last, a practical solution is provided to generate the worst few-shot set. All proofs are available in the Appendix~\ref{appendix:proof}.


%  \subsection{Few-shot Robustness Evaluation with MMD Maximization}
 
% To find the worst-case few-shot set, our goal is to solve the optimization problem stated in Eq.~\ref{main def}. Intuitively, the generalization errors increase when there are fewer correlations and lower distribution similarity between the few-shot set and test set. In many benchmarks and contests, the test set is not directly available, but we can use a well-rounded training set as a resource of natural data distribution. In this case, our optimization goal becomes maximizing the distribution distance between the few-shot set and original training set. Here we use MMD distance following \cite{gretton2012kernel}.



% \begin{definition} \label{def mmd}\textit{(Distribution Distance)}
%     Let $\mathcal{H}$ be the family of mappings from $\mathcal{X}\rightarrow \mathbbm{R^d}$, and let $P$ and $Q$ be two distribution,
%     then the MMD distance can be defined as, 
%     \begin{equation}
%         \text{MMD}(H, P,Q) := \sup_{f\in \mathcal{H}}(E_{x\sim P}[ f(x)] - E_{y\sim Q}[ f(y)]).
%     \end{equation}
% \end{definition}

% We theoretically show that the MMD distance is an upperbound for the few-shot robustness metric. 

% \begin{theorem}\label{covariate shift}\textit{(Few-shot Robustness Measured by MMD Discrepancy) } Let $\mathcal{H}$ be the hypothesis space $X\rightarrow \mathbbm{R^d}$. $f_{I_k}$ is the empirical risk $\epsilon_{P_{I_k}}(f)$ minimizer, and $f$ is the hypothesis that minimizes expected risk $\epsilon_{Q}(f)$. Then 
%     \begin{equation}
%     \epsilon_Q(f_{I_k}) \leq \epsilon_Q(f) + \text{MMD}(P_{I_k}, P) + \epsilon_{\alpha} + t + \epsilon_{\mathcal{H}},
% \end{equation}
% where $\epsilon_{\alpha}$,$t$ and $\epsilon_{H}$ are small constants describing the error occurred in training, the sampling behavior of training distribution and the hypothesis space complexity. Details are shown in Appendix~\ref{proof for cov}
% \end{theorem}

% % Therefore, when we want to solve the problem stated in Equation \ref{main def}, we look at few shot samples with a severe distribution shift.


% This theorem gives the intuition that a high discrepancy between the few-shot set and a training set results in high expected risk. Following statistics literature \citep{cheng2021neural}, a biased empirical estimate of the MMD is obtained by replacing the population expectations with the empirical average computed on the samples. Then we have,
% \begin{equation}
%     \text{MMD}(\mathcal{H}, P, P_{I_k}) := \sup_{f\in \mathcal{H}}(\frac{1}{n}\sum_{i=1}^n f(x_i) - \frac{1}{m}\sum_{m=1}^{k}f(x_{i_m}))
% \end{equation}

% For over-parameterized non-linear models, calculating MMD in the hypothesis space is intractable. Neural Tangent Kernel (NTK), however, is a simple approximation to understand neural networks as a kernel regression that can be optimized in its Reproducing Kernel Hilbert Space. 
% Following the convention in NTK literature, we consider the NTK kernel function defined for optimization step $t \ge 0$ as:
% \begin{equation}
%     K^t(x, x') := \langle\nabla_\theta f(\theta(t), x), \nabla_\theta f(\theta(t), x')\rangle.
% \end{equation}

% Then the MMD distance could be deducted following kernel conventions~\citep{gretton2012kernel}.

% \begin{proposition}\label{ntk-mmd def}
    
% \textit{(NMMD Distance)} The MMD static with NTK at time $t$ is, 
%     \begin{equation}
%     \text{MMD}^2_{K^t}(P, Q) = \int_{\mathcal{X}}\int_\mathcal{X'} K^t(x,x')(\hat p - \hat p')(x)(\hat p - \hat p')(x')dx dx',
% \end{equation}
% where $\mathcal{X}$ and $\mathcal{X'}$ denotes the support set for $P$ and $Q$.
% \end{proposition}

% When the neural network approaches its infinite width limit, the NTK matrix stays constant during training~\citep{arora2019exact, du2019gradient}, i.e., $K^t $ equals to $K^0$. This property enables us to accurately estimate the MMD distance without costly training. Together with the approximate ability of NTK for neural network training (shown in Proposition.~\ref{ntk}), we show that NMMD can be used as an approximation to the MMD distance.


% \begin{theorem} \label{mmd appx}\textit{(NMMD Approximation)} Let $\text{MMD}_f$ be the MMD distance calculated with model $f \in \mathcal{H}$ and let $\text{MMD}_K$ be the MMD static w.r.t. the NTK kernel $K$. Assume $f$ has taken $t$ steps of training at a learning rate of $\eta$, and $f$ is $L_f$-Lipschitz Continuous. Denote NTK at initialization as $K(x,x')= \langle\nabla_\theta f(\theta(0), x), \nabla_\theta f(\theta(0), x)\rangle$. If $k\leq \frac{n}{2}$, then the two MMD statistics satisfies: 
%    \begin{equation}
%     \text{MMD}_f(P,P_{I_k})) =O( t\eta\cdot \text{MMD}_{K}^2(P,P_{I_k}))
%    \end{equation}
% \end{theorem}
% This theorem formally justifies using NTK kernel to calculate MMD distances. Compared with estimating MMD distance with neural networks, this method requires no training, and its calculation can be easily decomposed into kernel similarity $K(x_i, x_j)$ with the help of the kernel trick. The simplified distance would be, 
% \begin{equation}
% \label{eq:mmdk}
%  \text{MMD}^2_K(P, P_{I_k}) = \frac{1}{n^2}\sum_{i,k}^n K(x_i, x_k) +  \underbrace{(\frac{1}{k^2}-\frac{2}{nk})\sum_{s,t}^k K(x_{i_s}, x_{i_t})}_{\text{intra-set kernel similarity}} - \underbrace{\frac{2}{nk}\sum_{i\in I_k, j\not \in I_k}K(x_i, x_j)}_{\text{inter-set kernel similarity}},
% \end{equation}
% This distance would achieve its maximum while maximizing the intra-set kernel similarity of the few-shot set and minimizing the inter-set kernel similarity.% between selected samples and others. 



==> 05_methodology.tex <==

\subsection{Implementation}
We have simplified the task of finding the worst few-shot set to maximizing the NMMD distance between a few-shot distribution and the full-size training distribution, as shown in Eq.~\ref{eq:mmdk}. However, there are several challenges in implementation: (1) The computational complexity for the NTK matrix on all training examples is $O(n^2)$, making it hard to scale to large-scale sets; (2) Optimizing the MMD distance requires solving a combinatorial problem of $O({n\choose k})$. In our work, we address these problems by taking advantage of the sparsity of NTK matrix. 

%, making it hard to scale to a sound number of training examples that creates a natural distribution of data

\paragraph{Efficient Optimization of Eq.~\ref{eq:mmdk}}

 In experiments, we discovered the NTK is usually a sparse, diagonally dominant matrix. As shown in Figure \ref{fig:ntkmat}, the diagonal terms $K(x_{i},x_{i})$ are more than 10x  larger than cross terms $K (x_{i},x_{j})$. In this way, we can discard cross terms for simplification in Eq.~\ref{eq:mmdk}. $K(x_{i},x_{i})$ is actually gradient norm $\langle \nabla_\theta{f(\theta, x_i)}, \nabla_\theta{f(\theta, x_i)}\rangle_{i\in[n]}$. 
Note that the gradient of model $f:\mathcal{X}\rightarrow \mathbbm{R}^d$ is $\nabla_{\theta}f(\theta(t),x)\in \mathbbm{R}_{p\times d}$, $p$ is the number of parameters in $f$. %When we calculate gradient norm, we aggregate both the parameter dimension as well as the label dimension \citep{arora2019exact}. 
The calculation of $K(x_{i},x_{i})$ can be written as, 
\begin{equation}
   K(x_{i},x_{i}) = \langle \nabla_\theta{f(\theta, x)}, \nabla_\theta{f(\theta, x)}\rangle = \sum_{i=1}^p \sum_{j=1}^d \nabla_{\theta_{i}}f_{j}(x)^2.
\end{equation}





%\textbf{Gradient Norm Ranking Approach}
After reducing the sparse terms in the NTK matrix, our new goal is to maximize the intra-set kernel similarity using the gradient norm terms:
\begin{equation}
    \max_{I_k}\sum_{s=1}^k K(x_{i_s}, x_{i_s}), i_s\in I_k
    \label{eq:finalob}
\end{equation}


\paragraph{Implementation Algorithm} Given Eq.~\ref{eq:finalob}, the target of finding the worst-case few-shot set is simplified into finding the few-shot set with the maximum sum gradient norms. The algorithm details are shown in Algorithm~\ref{alg:algorithm}. First, 
We rank all training samples w.r.t. their gradient norms, i.e., $K(x_{j_1},x_{j_1}) > K(x_{j_2},x_{j_2})> ...> K(x_{j_n},x_{j_n}) $, then we choose the top-k samples $(x_{j_s},y_{j_s})_{s\in [k]}$ as our attack few-shot set. Last, we train models on the searched few-shot set and report its test accuracy. 


\begin{figure}
    \begin{minipage}[b]{0.5\textwidth}
      \begin{algorithm}[H]
 \textbf{Input}: Full-size training set $X = (x_i, y_i)_{i=1}^n$, few-shot set size $k$, model $f$ with random parameters $\theta$, initial parameters $\theta_0$.
 
 \textbf{Output}: The few-shot attack set. 
 
 \begin{algorithmic}[1] %[1] enables line numbers
  \STATE Initialize $f_{\theta}$ with  $\theta_0$
  \FOR {$i=1:n$}
  \STATE $G_i \leftarrow \langle \nabla_{\theta}f_{\theta}(x_i), \nabla_{\theta}f_{\theta}(x_i)\rangle$
  \ENDFOR
  \STATE Sort examples in X based on $G_i$ %X$\leftarrow$ sort($X$, key=$G$)
  \STATE For each label, select top $k$ examples into \\the final few-shot set $\text{X}_{\text{few}}$ to optimize Eq.~\ref{eq:finalob}
  %\STATE $\text{X}_{\text{few}} \leftarrow \{\text{x}_i\}_{i=1}^k$
 \RETURN $\text{X}_{\text{few}}$
 \end{algorithmic}
 
 \caption{Details of NMMD-Attack. }
  \label{alg:algorithm}
\end{algorithm}
    \end{minipage}
    \begin{minipage}[b]{\linewidth}
        \centering
        \includegraphics[scale=0.4]{image/heatmap1.jpg}
        \caption{Visualization of NTK matrix with 50 examples randomly sampled from CIFAR-10. }
    %, while the matrix is average of 5 matrix All the 500 samples are randomly sampled from CIFAR10. NTK matrix is sparse. 
    \label{fig:ntkmat}
    \end{minipage}
    
\end{figure}


==> tables/04_nlp_5000_shot.tex <==

 \begin{table*}[htbp!]
	\centering
	\caption{
		The 5000 shot results on GLUE. The abbreviations follow Table 1.
	}
    \footnotesize
	% \resizebox{0.9\textwidth}{!}{%
		\begin{tabular}{ll|c|cc|cc}
			\toprule
\multirow{2}{*}{\textbf{Datasets}}   & \multirow{2}{*}{\textbf{Models}} & \multirow{1}{*}{\textbf{\methodRandom}} & \multicolumn{2}{c|}{\textbf{\methodgd }} & \multicolumn{2}{c}{\textbf{\methodls}} \\

   % \cmidrule(lr){3-3}  \cmidrule(lr){4-5} \cmidrule(lr){6-7}
 %  \cmidrule(lr){3-4}  \cmidrule(lr){5-6} \cmidrule(lr){7-8}
   & & \textbf{Accuracy} & \textbf{Accuracy} & \textbf{Gap} & \textbf{Accuracy} & \textbf{Gap} \\
			\midrule
    
   \multirow{5}{*}{SST2}
& Transformer &  77.66\std{  0.91} &   57.29\std{  1.00} & \gap{ 20.37} &  56.72\std{  0.75} & \gap{ 20.94}  \\
& BERT        &  91.95\std{  0.33} &   67.82\std{  3.14} & \gap{ 24.13} &  69.86\std{  1.68} & \gap{ 22.09}  \\
& GPT-2        &  91.12\std{  0.70} &   76.06\std{  1.90} & \gap{ 15.06} &  71.70\std{  1.21} & \gap{ 19.42}  \\
& RoBERTa     &  93.19\std{  0.21} &   88.17\std{  0.81} & \gap{  5.02} &  88.35\std{  0.69} & \gap{  4.84}  \\
& T5          &  91.51\std{  1.14} &   87.89\std{  1.08} & \gap{  3.62} &  88.67\std{  0.35} & \gap{  2.84}  \\
\midrule

\multirow{5}{*}{MNLI matched}
& Transformer &  44.28\std{  0.34} &   35.18\std{  0.53} & \gap{  9.10} &  33.98\std{  1.22} & \gap{ 10.30}  \\
& BERT        &  73.01\std{  0.23} &   31.05\std{  1.45} & \gap{ 41.96} &  18.44\std{  0.59} & \gap{ 54.57}  \\
& GPT-2        &  71.90\std{  0.50} &   33.55\std{  1.21} & \gap{ 38.35} &  25.57\std{  1.82} & \gap{ 46.33}  \\
& RoBERTa     &  82.11\std{  0.28} &   38.99\std{  0.74} & \gap{ 43.12} &  14.97\std{  0.58} & \gap{ 67.14}  \\
& T5          &  78.93\std{  0.31} &   33.11\std{  0.61} & \gap{ 45.82} &  31.96\std{  0.52} & \gap{ 46.97}  \\

\midrule

\multirow{5}{*}{MNLI mismatched}
& Transformer &  45.72\std{  0.32} &   34.98\std{  0.48} & \gap{ 10.74} &  33.82\std{  1.19} & \gap{ 11.90}  \\
& BERT        &  74.13\std{  0.28} &   29.93\std{  1.88} & \gap{ 44.20} &  17.11\std{  0.76} & \gap{ 57.02}  \\
& GPT-2        &  73.61\std{  0.42} &   32.96\std{  1.66} & \gap{ 40.65} &  26.09\std{  2.04} & \gap{ 47.52}  \\
& RoBERTa     &  82.51\std{  0.18} &   36.82\std{  1.08} & \gap{ 45.69} &  13.99\std{  0.60} & \gap{ 68.52}  \\
& T5          &  79.43\std{  0.31} &   33.34\std{  0.80} & \gap{ 46.09} &  31.84\std{  0.53} & \gap{ 47.59}  \\
\midrule

\multirow{5}{*}{QNLI}
& Transformer &  58.84\std{  0.27} &   52.26\std{  0.52} & \gap{  6.58} &  50.22\std{  0.64} & \gap{  8.62}  \\
& BERT        &  84.10\std{  0.84} &   36.09\std{  3.52} & \gap{ 48.01} &  24.07\std{  0.74} & \gap{ 60.03}  \\
& GPT-2        &  82.72\std{  0.51} &   50.04\std{  2.65} & \gap{ 32.68} &  39.92\std{  5.55} & \gap{ 42.80}  \\
& RoBERTa     &  89.21\std{  0.31} &   34.23\std{  1.09} & \gap{ 54.98} &  22.09\std{  1.66} & \gap{ 67.12}  \\
& T5          &  88.52\std{  0.24} &   48.86\std{  1.14} & \gap{ 39.66} &  42.29\std{  2.24} & \gap{ 46.23}  \\
\midrule

\multirow{5}{*}{QQP}
& Transformer &  71.05\std{  0.65} &   58.38\std{  3.82} & \gap{ 12.67} &  42.23\std{  2.98} & \gap{ 28.82}  \\
& BERT        &  81.74\std{  0.26} &   39.49\std{  1.54} & \gap{ 42.25} &  23.37\std{  0.40} & \gap{ 58.37}  \\
& GPT-2        &  81.55\std{  0.36} &   49.28\std{  4.25} & \gap{ 32.27} &  28.51\std{  1.42} & \gap{ 53.04}  \\
& RoBERTa     &  84.82\std{  0.18} &   40.25\std{  3.42} & \gap{ 44.57} &  19.60\std{  0.62} & \gap{ 65.22}  \\
& T5          &  85.62\std{  0.14} &   54.78\std{  2.43} & \gap{ 30.84} &  33.39\std{  0.79} & \gap{ 52.23}  \\

\bottomrule
		\end{tabular}%
	% }
	\vspace{-0.5ex}
	\label{tab:04_nlp_5000}
\end{table*} 



%  \begin{table*}[t!]
% 	\centering
% 	\caption{
% 		The 5000 shot comparisons between average performance and attack (FFN-attack) performance on GLUE. The abbreviations follow Table 1.
% 	}
%     \footnotesize
% 	\resizebox{0.8\textwidth}{!}{%
% 		\begin{tabular}{llrrrrrr}
% 			\toprule
% \multirow{2}{*}{\textbf{Datasets}}   & \multirow{2}{*}{\textbf{Models}} & \multicolumn{2}{c}{\textbf{Average-case}} & \multicolumn{2}{c}{\textbf{\method }} & \multicolumn{2}{c}{\textbf{Loss-based}} \\

%     \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
%    &  &   \textbf{Train Acc.} & \textbf{Test Acc.} & \textbf{Train Acc.} & \textbf{Test  Acc.} & \textbf{Train Acc.} & \textbf{Test  Acc.} \\ 
% 			\midrule
  
%    \multirow{5}{*}{SST2}
% & Transformer&  96.55\std{0.19} &  77.66\std{0.91} &  90.01\std{0.60} &  57.29\std{1.00} &  90.27\std{0.32} &  56.72\std{0.75} \\
% & BERT       &  99.47\std{0.07} &  91.95\std{0.33} &  97.50\std{0.08} &  67.82\std{3.14} &  97.41\std{0.12} &  69.86\std{1.68} \\
% & GPT-2       &  98.12\std{0.11} &  91.12\std{0.70} &  89.14\std{0.86} &  76.06\std{1.90} &  89.10\std{1.17} &  71.70\std{1.21} \\
% & RoBERTa    &  98.86\std{0.07} &  93.19\std{0.21} &  94.22\std{0.35} &  88.17\std{0.81} &  94.64\std{0.20} &  88.35\std{0.69} \\
% & T5         &  96.16\std{1.08} &  91.51\std{1.14} &  82.11\std{0.39} &  87.89\std{1.08} &  82.96\std{0.23} &  88.67\std{0.35} \\
% \midrule
   
% \multirow{5}{*}{MNLI matched}
% & Transformer&  83.98\std{2.41} &  44.28\std{0.34} &  42.03\std{13.22} &  35.18\std{0.53} & ???.??\std{?.??} & ???.??\std{?.??} \\
% & BERT       &  98.57\std{0.11} &  73.01\std{0.23} &  97.86\std{0.29} &  31.05\std{1.45} &  97.67\std{0.11} &  18.44\std{0.59} \\
% & GPT-2       &  93.04\std{0.48} &  71.90\std{0.50} &  72.87\std{3.28} &  33.55\std{1.21} &  81.50\std{1.20} &  25.57\std{1.82} \\
% & RoBERTa    &  98.08\std{0.11} &  82.11\std{0.28} &  95.34\std{0.13} &  38.99\std{0.74} &  95.29\std{0.30} &  14.97\std{0.58} \\
% & T5         &  88.84\std{0.30} &  78.93\std{0.31} &  59.86\std{0.47} &  33.11\std{0.61} &  66.74\std{1.13} &  31.96\std{0.52} \\

% \midrule
   
% \multirow{5}{*}{MNLI mismatched}
% & Transformer&  83.77\std{1.49} &  45.72\std{0.32} &  42.03\std{13.22} &  34.98\std{0.48} &  83.25\std{1.20} &  33.82\std{1.19} \\
% & BERT       &  98.56\std{0.09} &  74.13\std{0.28} &  97.86\std{0.29} &  29.93\std{1.88} &  97.67\std{0.11} &  17.11\std{0.76} \\
% & GPT-2       &  92.82\std{0.28} &  73.61\std{0.42} &  72.87\std{3.28} &  32.96\std{1.66} &  81.50\std{1.20} &  26.09\std{2.04} \\
% & RoBERTa    &  97.94\std{0.08} &  82.51\std{0.18} &  95.34\std{0.13} &  36.82\std{1.08} &  95.29\std{0.30} &  13.99\std{0.60} \\
% & T5         &  88.66\std{0.55} &  79.43\std{0.31} &  59.86\std{0.47} &  33.34\std{0.80} &  66.74\std{1.13} &  31.84\std{0.53} \\
% \midrule
   
% \multirow{5}{*}{QNLI}
% & Transformer&  96.54\std{0.19} &  58.84\std{0.27} &  96.60\std{0.22} &  52.26\std{0.52} &  95.88\std{0.61} &  50.22\std{0.64} \\
% & BERT       &  99.03\std{0.21} &  84.10\std{0.84} &  98.58\std{0.18} &  36.09\std{3.52} &  99.06\std{0.05} &  24.07\std{0.74} \\
% & GPT-2       &  95.66\std{0.19} &  82.72\std{0.51} &  91.22\std{1.80} &  50.04\std{2.65} &  94.27\std{0.99} &  39.92\std{5.55} \\
% & RoBERTa    &  98.68\std{0.10} &  89.21\std{0.31} &  97.47\std{0.20} &  34.23\std{1.09} &  98.03\std{0.14} &  22.09\std{1.66} \\
% & T5         &  96.02\std{0.23} &  88.52\std{0.24} &  83.33\std{0.85} &  48.86\std{1.14} &  89.53\std{0.53} &  42.29\std{2.24} \\
% \midrule
   
% \multirow{5}{*}{QQP}
% & Transformer&  93.55\std{0.50} &  71.05\std{0.65} &  92.69\std{0.27} &  58.38\std{3.82} &  92.97\std{0.47} &  42.23\std{2.98} \\
% & BERT       &  98.80\std{0.11} &  81.74\std{0.26} &  98.70\std{0.11} &  39.49\std{1.54} &  99.35\std{0.07} &  23.37\std{0.40} \\
% & GPT-2       &  94.48\std{0.85} &  81.55\std{0.36} &  91.51\std{1.45} &  49.28\std{4.25} &  96.66\std{0.44} &  28.51\std{1.42} \\
% & RoBERTa    &  98.27\std{0.20} &  84.82\std{0.18} &  97.70\std{0.15} &  40.25\std{3.42} &  98.70\std{0.20} &  19.60\std{0.62} \\
% & T5         &  94.83\std{0.47} &  85.62\std{0.14} &  84.49\std{0.67} &  54.78\std{2.43} &  96.27\std{0.26} &  33.39\std{0.79} \\

% \bottomrule
% 		\end{tabular}%
% 	}
% 	\vspace{-0.5ex}
% 	\label{tab:main}
% \end{table*} 


==> tables/06_ood_nlp.tex <==

 \begin{table*}[htbp]
	\centering
	\caption{
		The out of distribution examination on GLUE. The abbreviations follow Table 1.
	}
    \footnotesize
	% \resizebox{0.9\textwidth}{!}{%
		\begin{tabular}{ll|c|cc|cc}
			\toprule
\multirow{2}{*}{\textbf{Datasets}}   & \multirow{2}{*}{\textbf{Models}} & \multirow{1}{*}{\textbf{\methodRandom}} & \multicolumn{2}{c|}{\textbf{\methodgd }} & \multicolumn{2}{c}{\textbf{\methodls}} \\

   % \cmidrule(lr){3-3}  \cmidrule(lr){4-5} \cmidrule(lr){6-7}
 %  \cmidrule(lr){3-4}  \cmidrule(lr){5-6} \cmidrule(lr){7-8}
   & & \textbf{Accuracy} & \textbf{Accuracy} & \textbf{Gap} & \textbf{Accuracy} & \textbf{Gap} \\
			\midrule
   
\multirow{5}{*}{SST2}
& Transformer &  90.03\std{  0.33} &  65.15\std{  0.43} & \gap{ 24.88} &  64.67\std{  0.54} & \gap{ 25.36}  \\
& BERT        &  94.96\std{  0.28} &  70.53\std{  0.47} & \gap{ 24.43} &  70.67\std{  0.25} & \gap{ 24.29}  \\
& GPT-2        &  93.88\std{  0.17} &  70.24\std{  0.23} & \gap{ 23.64} &  69.84\std{  0.45} & \gap{ 24.04}  \\
& RoBERTa     &  94.71\std{  0.25} &  73.69\std{  0.52} & \gap{ 21.02} &  73.33\std{  0.34} & \gap{ 21.38}  \\
& T5          &  95.55\std{  0.15} &  77.16\std{  0.33} & \gap{ 18.39} &  76.68\std{  0.24} & \gap{ 18.87}  \\
\midrule

\multirow{5}{*}{COLA}
& Transformer &  70.45\std{  0.00} &  70.45\std{  0.00} & \gap{  0.00} &  70.45\std{  0.00} & \gap{  0.00}  \\
& BERT        &  83.48\std{  0.61} &  53.48\std{  1.33} & \gap{ 30.00} &  49.51\std{  1.96} & \gap{ 33.97}  \\
& GPT-2        &  77.96\std{  0.68} &  69.23\std{  0.96} & \gap{  8.73} &  69.35\std{  0.55} & \gap{  8.61}  \\
& RoBERTa     &  85.44\std{  0.85} &  61.81\std{  0.61} & \gap{ 23.63} &  57.89\std{  1.37} & \gap{ 27.55}  \\
& T5          &  83.64\std{  0.70} &  70.45\std{  0.00} & \gap{ 13.19} &  70.45\std{  0.00} & \gap{ 13.19}  \\
\midrule

\multirow{5}{*}{MNLI matched}
& Transformer &  59.63\std{  0.53} &  33.27\std{  0.10} & \gap{ 26.36} &  31.92\std{  0.18} & \gap{ 27.71}  \\
& BERT        &  82.87\std{  0.26} &  34.54\std{  0.36} & \gap{ 48.33} &  31.27\std{  0.58} & \gap{ 51.60}  \\
& GPT-2        &  81.42\std{  0.13} &  38.35\std{  0.25} & \gap{ 43.07} &  35.18\std{  0.40} & \gap{ 46.24}  \\
& RoBERTa     &  86.70\std{  0.11} &  47.03\std{  0.47} & \gap{ 39.67} &  43.74\std{  0.46} & \gap{ 42.96}  \\
& T5          &  86.73\std{  0.13} &  48.82\std{  0.36} & \gap{ 37.91} &  45.27\std{  0.46} & \gap{ 41.46}  \\
\midrule

\multirow{5}{*}{MNLI mismatched}
& Transformer &  59.84\std{  0.76} &  33.28\std{  0.10} & \gap{ 26.56} &  31.92\std{  0.18} & \gap{ 27.92}  \\
& BERT        &  82.68\std{  0.15} &  34.54\std{  0.36} & \gap{ 48.14} &  31.27\std{  0.58} & \gap{ 51.41}  \\
& GPT-2        &  81.32\std{  0.22} &  38.35\std{  0.25} & \gap{ 42.97} &  35.18\std{  0.40} & \gap{ 46.14}  \\
& RoBERTa     &  86.53\std{  0.13} &  47.03\std{  0.47} & \gap{ 39.50} &  43.74\std{  0.46} & \gap{ 42.79}  \\
& T5          &  86.70\std{  0.14} &  48.82\std{  0.36} & \gap{ 37.88} &  45.27\std{  0.46} & \gap{ 41.43}  \\
\midrule

\multirow{5}{*}{QNLI}
& Transformer &  59.97\std{  0.53} &  51.51\std{  0.24} & \gap{  8.46} &  47.92\std{  0.27} & \gap{ 12.05}  \\
& BERT        &  87.80\std{  0.66} &  51.03\std{  0.47} & \gap{ 36.77} &  45.51\std{  1.05} & \gap{ 42.29}  \\
& GPT-2        &  86.36\std{  0.24} &  52.98\std{  0.47} & \gap{ 33.38} &  47.16\std{  0.29} & \gap{ 39.20}  \\
& RoBERTa     &  90.81\std{  0.10} &  59.74\std{  0.31} & \gap{ 31.07} &  54.46\std{  0.30} & \gap{ 36.35}  \\
& T5          &  90.90\std{  0.16} &  60.20\std{  0.32} & \gap{ 30.70} &  55.39\std{  0.21} & \gap{ 35.51}  \\
\midrule

\multirow{5}{*}{MRPC}
& Transformer &  69.64\std{  0.59} &  67.49\std{  0.00} & \gap{  2.15} &  67.49\std{  0.00} & \gap{  2.15}  \\
& BERT        &  81.45\std{  1.60} &  65.98\std{  0.61} & \gap{ 15.47} &  30.19\std{  4.89} & \gap{ 51.26}  \\
& GPT-2        &  79.32\std{  1.58} &  65.79\std{  0.77} & \gap{ 13.53} &  45.74\std{  8.00} & \gap{ 33.58}  \\
& RoBERTa     &  86.07\std{  0.56} &  77.38\std{  0.68} & \gap{  8.69} &  49.45\std{  2.38} & \gap{ 36.62}  \\
& T5          &  81.37\std{  0.66} &  67.62\std{  0.27} & \gap{ 13.75} &  67.46\std{  0.06} & \gap{ 13.91}  \\
\midrule

\multirow{5}{*}{QQP}
& Transformer &  79.80\std{  0.31} &  55.42\std{  1.09} & \gap{ 24.38} &  54.15\std{  0.86} & \gap{ 25.65}  \\
& BERT        &  90.18\std{  0.07} &  50.76\std{  0.62} & \gap{ 39.42} &  48.78\std{  0.97} & \gap{ 41.40}  \\
& GPT-2        &  89.09\std{  0.16} &  51.32\std{  0.66} & \gap{ 37.77} &  49.65\std{  0.71} & \gap{ 39.44}  \\
& RoBERTa     &  90.83\std{  0.18} &  55.52\std{  0.70} & \gap{ 35.31} &  53.19\std{  0.33} & \gap{ 37.64}  \\
& T5          &  92.41\std{  0.13} &  59.52\std{  0.46} & \gap{ 32.89} &  57.77\std{  0.35} & \gap{ 34.64}  \\
\midrule

\multirow{5}{*}{RTE}
& Transformer &  50.38\std{  0.56} &  50.10\std{  0.00} & \gap{  0.28} &  50.10\std{  0.00} & \gap{  0.28}  \\
& BERT        &  61.53\std{  1.19} &  47.20\std{  1.24} & \gap{ 14.33} &  36.90\std{  2.75} & \gap{ 24.63}  \\
& GPT-2        &  66.40\std{  3.00} &  54.33\std{  1.75} & \gap{ 12.07} &  48.97\std{  1.40} & \gap{ 17.43}  \\
& RoBERTa     &  76.18\std{  1.59} &  65.79\std{  2.24} & \gap{ 10.39} &  60.12\std{  1.04} & \gap{ 16.06}  \\
& T5          &  56.98\std{  0.96} &  48.65\std{  2.43} & \gap{  8.33} &  47.00\std{  2.84} & \gap{  9.98}  \\
\midrule

\multirow{5}{*}{WNLI}
& Transformer &  50.79\std{  0.00} &  50.79\std{  0.00} & \gap{  0.00} &  50.79\std{  0.00} & \gap{  0.00}  \\
& BERT        &  45.87\std{  4.03} &  46.98\std{  5.82} & \gap{ -1.11} &  30.32\std{  7.55} & \gap{ 15.55}  \\
& GPT-2        &  47.78\std{  1.77} &  49.68\std{  1.63} & \gap{ -1.90} &  52.22\std{  4.12} & \gap{ -4.44}  \\
& RoBERTa     &  50.95\std{  0.32} &  50.79\std{  0.00} & \gap{  0.16} &  50.79\std{  0.00} & \gap{  0.16}  \\
& T5          &  49.21\std{  1.12} &  48.73\std{  0.95} & \gap{  0.48} &  48.41\std{  2.01} & \gap{  0.80}  \\

\bottomrule
		\end{tabular}%
	% }
	\vspace{-0.5ex}
	\label{tab:main}
\end{table*} 


==> tables/07_cv_mixup.tex <==
\begin{table}[ht]
\centering
\caption{
    Results with cutmix. Both of \BenchName keep the gap compared to \methodRandom.
}
\label{tab:dataaug}
     \footnotesize
  \resizebox{\linewidth}{!}{%
		\begin{tabular}{l|ccc}
			\toprule
\textbf{Models} & \textbf{\methodRandom} & \textbf{\methodgd} & \textbf{\methodls} \\
\midrule

 
 FFN              &  50.97\std{0.72} &  29.37\std{0.82} &  17.73\std{0.32} \\
 VGG-16           &  64.72\std{0.61} &  46.88\std{0.66} &  31.53\std{0.68} \\
 ResNet-18        &  65.46\std{0.69} &  51.27\std{1.42} &  34.73\std{0.39} \\
 DenseNet-121     &  75.13\std{0.69} &  62.28\std{1.83} &  45.97\std{3.22} \\
 ViT-B/16         &  97.25\std{0.11} &  97.66\std{0.09} &  96.91\std{0.18} \\
 EfficientNetV2-S & 91.22\std{?.??} &  90.08\std{1.87} &  89.29\std{0.67} \\
			\bottomrule
		\end{tabular}
 }

\end{table}

